Absolute frequency measurement of the 1S0 - 3P0 transition of 171Yb

We report the absolute frequency measurement of the unperturbed transition 1S0 - 3P0 at 578 nm in 171Yb realized in an optical lattice frequency standard. The absolute frequency is measured 518 295 836 590 863.55(28) Hz relative to a cryogenic caesium fountain with a fractional uncertainty of 5.4x10-16 . This value is in agreement with the ytterbium frequency recommended as a secondary representation of the second in the International System of Units.

==> pictures/levels.tikz.tex <==
\begin{tikzpicture}
	[
	level/.style={black, thick},
	shiftl/.style={gray, semithick},
	transition/.style={very thick, ->,},
	block/.style={rectangle, fill=#1!10!white, text=black},
	>=stealth, yscale=0.25, xscale=.35, 
	]

\footnotesize


%seaborn deep palette color
\definecolor{blue}{rgb}{0.2980392156862745, 0.4470588235294118, 0.6901960784313725}
\definecolor{green}{rgb}{0.3333333333333333, 0.6588235294117647, 0.40784313725490196}
\definecolor{red}{rgb}{0.7686274509803922, 0.3058823529411765, 0.3215686274509804}
\definecolor{purple}{rgb}{0.5058823529411764, 0.4470588235294118, 0.6980392156862745}
\definecolor{yellow2}{rgb}{0.8, 0.7254901960784313, 0.4549019607843137}


\draw[transition, blue] (-0.5,2) -- node[block=blue,auto, align=center, font=\footnotesize, near end] {$\lambda\!=\!\SI{399}{nm}$\\$\Gamma/2\pi\!=\!\SI{29}{MHz}$} (-2,25);
\draw[transition, green!100!black] (1.5,2) -- node[block=green,auto, align=center, font=\footnotesize, pos=0.55] {$\lambda\!=\!\SI{556}{nm}$\\$\Gamma/2\pi\!=\!\SI{182}{kHz}$} (3.5,18.0);
%\draw[transition, yellow!100!black] (2.5,2) -- node[block=yellow,auto, swap, align=center, font=\footnotesize, near end] {$\lambda\!=\!\SI{578}{nm}$\\$\Gamma\!<\!\SI{10}{mHz}$} (4.5,17.3);


\draw[transition, yellow!50!yellow2] (9,1) -- node[block=yellow,auto, align=center, font=\footnotesize, swap] {$\lambda\!=\!\SI{578}{nm}$\\$\Gamma/2\pi\!<\!\SI{10}{mHz}$} (12,16.0);
\draw[transition, yellow!50!yellow2] (8,-1) --  (11,14.0);


\draw[transition, red!80!gray] (5.5,17.0) -- node[block=red!80!gray,auto, align=center, font=\footnotesize, pos=0.65] {$\lambda\!=\!\SI{1389}{nm}$\\$\Gamma/2\pi\!=\!\SI{483}{kHz}$} (5.5,24.4);

\node[block=red,align=center,font=\footnotesize] (magic) at (3.2,-3) {lattice $\lambda\ped{magic}\!=\!\SI{759}{nm}$};
\draw[->,out=90, in=250] (magic) to (3.7, 0.6);
\draw[->, out=90, in=250] (magic) to (6.5, 16.0);


\draw[level] (-1,2)-- (3,2) ; % sarebbe 0 %  node[left] {\ch{^1S0}} 
\draw[level] (-3,25) node[left] {\ch{^1P1}} -- (1,25) ;
\draw[level] (2,19.7)  -- (6,19.7) node[anchor=195] {\ch{^3P2}} ;
\draw[level] (2,18.0)  -- (6,18.0) node[anchor=195] {\ch{^3P1}} ;
\draw[level] (2,17.0)-- (6,17.0) ; %sarebbe 17.3 % node[anchor=15] {\ch{^3P0}} 

\draw[level] (3,25.5) --  (7,25.5) node[anchor=205] {\ch{^3D3}}; %sarebbe 25.3
\draw[level] (3,24.9) -- (7,24.9) node[right] {\ch{^3D2}};% sarebbe 24.8, 
\draw[level] (3,24.4) -- (7,24.4) node[anchor=150] {\ch{^3D1}};% sarebbe 24.5


\draw[level] (7,15.0) -- node[above] {\ch{^3P0}} (9,15.0) ; %3P0 shifted
\draw[level] (4,0)-- node[above] {\ch{^1S0}} (6,0) ; %1S0 shifted

\
\draw[level] (10,16.0) -- (13,16.0) node[right] {$m_F\!=\!\frac{1}{2}$};; %3P0 splitted
\draw[level] (10,14.0) -- (13,14.0) node[right] {$m_F\!=\!-\frac{1}{2}$};; %3P0 splitted
\draw[level] (7,1)-- (10,1) node[right] {$m_F\!=\!\frac{1}{2}$}; %1S0 shifted
\draw[level] (7,-1)-- (10,-1) node[right] {$m_F\!=\!-\frac{1}{2}$}; %1S0 shifted


\draw[shiftl] (3,2) -- (4,0);
\draw[shiftl] (6,17.0) -- (7,15.0);


\draw[shiftl] (9,15.0) -- (10,16.0);
\draw[shiftl] (9,15.0) -- (10,14.0);
\draw[shiftl] (6,0) -- (7,1);
\draw[shiftl] (6,0) -- (7,-1);


\end{tikzpicture}


==> table.tex <==
\begin{table*}
\caption{Uncertainty budget for the Yb-ITCsF2 Comparison}
\label{tab:budget}
\centering
\begin{tabular}{lSSSS}
\br
Effect 	&{Shift. /Hz}	&{Unc./Hz}		&{Shift.$\times$\num{e16}}	&{Unc.$\times$\num{e16}}\\
\mr
{Zeeman shift}	&-0.14	&0.02	&-2.7	&0.4\\
{Polarizability} 	&-0.04	&0.04	&-0.8	&0.8\\
{Hyperpolarizability} 	&0.026	&0.006	&0.50	&0.12\\
{Multipolar effects} 	&0.00	&{?}	&0.0	&{?}\\
{BBR room} 		&-1.219	&0.013	&-23.52	&0.25\\
{BBR oven} 		&-0.011	&0.004	&-0.21	&0.08\\
{Density shift} 	&-0.01	&0.03	&-0.2	&0.6\\
{Probe light shift} 	&0.0027	&0.0012	&0.05	&0.02\\
{Background gas shift} 	&0.00	&{?}	&0.0	&{?}\\
{dc Stark shift} 	&0.00	&{?}	&0.0	&{?}\\
{Line pulling} 	&0.00	&{?}	&0.0	&{?}\\
{Servo error} 	&0.00	&{?}	&0.0	&{?}\\
{Tunnelling} 	&0.00	&{?}	&0.0	&{?}\\
{AOM phase chirp} 	&0.00	&{?}	&0.0	&{?}\\
{Gravitational redshift} &13.474	&0.002	&260.12	&0.04\\
\mr
\textbf{Total Yb}	&?	&0.06	&?	&1.3\\
\mr
{Fiber links} 	&0.00	&{?}	&0.0	&{?}\\
{Synchronization} 	&0.00	&{?}	&0.0	&{?}\\
{Comb}		&0.00	&{?}	&0.0	&{?}\\
{Statistical}	&{--}	&0.18	&{--}	&3.4\\
{ITCsF2 syst}	&{--}	&0.2	&{--}	&3.9\\
{ITCSF2 redshift} 	&{?}	&0.002	&{?}	&0.04\\
\mr
\textbf{Total} 	&?	&0.28	&?	&5.4\\
\br
\end{tabular}
\end{table*}

